On the estimation of specific interfacial areas in aerated flows

This work provides a short clarification on the definition of specific interfacial areas in aerated flows, thereby distinguishing between the specific interfacial area related to the volume of an air-water mixture, and the specific interfacial area related to the water volume. This distinction is important when it comes to solving the air-water mass transfer equation, as there has been some misconception on the past. It is hoped that this contribution will help to clarify on these basic fundamentals, which is anticipated to be important for the future development and application of advanced air-water mass transfer models to aerated flows.

==> Figures/Fig1.tex <==
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 1, horizontal sep=1.85 cm, vertical sep=1.5cm},height=6.5 cm,width=6.5 cm,
  legend style={at={(1.1,  1)},anchor=north west},xmajorgrids=true,ymajorgrids=true,]


\nextgroupplot[xlabel=$C$,ylabel= $y/y_{90}$,xmin=0,xmax=1,ymin=0,ymax=2,title=(\textbf{a})]

\draw [black, draw opacity=0, name path=C] plot [smooth, tension=0] coordinates {(0,0) (1,0)};
\draw [black, draw opacity=0, name path=D] plot [smooth, tension=0] coordinates {(0,0.4) (1,0.4)};
\addplot+[blue, opacity=0.1] fill between[of=C and D]; 

\draw [black, draw opacity=0, name path=C] plot [smooth, tension=0] coordinates {(0,0.4) (1,0.4)};
\draw [black, draw opacity=0, name path=D] plot [smooth, tension=0] coordinates {(0,0.74) (1,0.74)};
\addplot+[violet, opacity=0.1] fill between[of=C and D]; 

\draw [black, draw opacity=0, name path=C] plot [smooth, tension=0] coordinates {(0,0.74) (1,0.74)};
\draw [black, draw opacity=0, name path=D] plot [smooth, tension=0] coordinates {(0,2) (1,2)};
\addplot+[cyan, opacity=0.1] fill between[of=C and D]; 


% filling
% color on the central part

\addplot [only marks, mark size = 3, fill=black, opacity=1, mark=*]
table{%	
0.061723333	0.011
0.108456667	0.076
0.142693333	0.141
0.168516667	0.206
0.202821111	0.272
0.258221667	0.338
0.30681	0.403
0.390986111	0.468
0.466738889	0.534
0.536447778	0.599
0.625359444	0.664
0.694188889	0.730
0.763385	0.795
0.811574444	0.861
0.864513333	0.926
0.896886111	0.991
0.9	1.000
0.919987778	1.056
0.937908333	1.122
0.955298889	1.187
0.962045	1.252
0.974681111	1.318
0.976736111	1.383
0.975732222	1.449
0.979264444	1.514
0.984131667	1.579
};


\nextgroupplot[xlabel=$a$ (1/m),ylabel= $y/y_{90}$,xmin=0,xmax=1000,ymin=0,ymax=2,title=(\textbf{b}),legend style={at={(-1.38,  1.25)},anchor=south west},legend columns=2] 



\addplot [only marks, mark size = 3, fill=black, opacity=1, mark=*]
table{%	
0 -1 
};\addlegendentry{$C$ \, }


\draw [black, draw opacity=0, name path=C] plot [smooth, tension=0] coordinates {(0,0.74) (1000,0.74)};
\draw [black, draw opacity=0, name path=D] plot [smooth, tension=0] coordinates {(0,2) (1000,2)};

\addplot+[cyan, opacity=0.1] fill between[of=C and D]; \addlegendentry{Droplet flow layer; $C > 0.7$} 


\addplot [only marks, mark size = 4, opacity=1, mark=diamond] table{%	
0 -1
}; \addlegendentry{$a_\text{m}$; Eq. (\ref{Eq1}) \, }


\draw [black, draw opacity=0, name path=C] plot [smooth, tension=0] coordinates {(0,0.4) (1000,0.4)};
\draw [black, draw opacity=0, name path=D] plot [smooth, tension=0] coordinates {(0,0.74) (1000,0.74)};
\addplot+[violet, opacity=0.1] fill between[of=C and D]; \addlegendentry{\, Intermediate flow layer; $0.3 \leq C \leq 0.7$} 

\addplot [only marks, mark size = 3, fill=blue, opacity=1, mark=*] table{%	
0 -1
}; \addlegendentry{$a_\text{w}$; Eq. (\ref{Eq9}) \, } 


 \draw [black, draw opacity=0, name path=C] plot [smooth, tension=0] coordinates {(0,0) (1000,0)};
\draw [black, draw opacity=0, name path=D] plot [smooth, tension=0] coordinates {(0,0.4) (1000,0.4)};
\addplot+[blue, opacity=0.15] fill between[of=C and D]; \addlegendentry{Bubbly flow layer; $C < 0.3$} 





\addplot [only marks, mark size = 4, opacity=1, mark=diamond] table{%	
-574.7006369	0.011
263.2318943	0.076
255.841472	0.141
267.9353621	0.206
276.3765039	0.272
287.4687426	0.338
294.3236612	0.403
297.5800896	0.468
289.7537155	0.534
274.210427	0.599
248.309507	0.664
215.8683652	0.730
171.8310922	0.795
146.836518	0.861
111.8150507	0.926
88.98702524	0.991
68.07643312	1.056
57.26822364	1.122
42.18164661	1.187
34.49681529	1.252
24.40764331	1.318
22.07643312	1.383
23.56687898	1.449
19.51592357	1.514
14.68789809	1.579
}; 


\addplot [only marks, mark size = 3, fill=blue, opacity=1, mark=*] table{%	
-612.5065851	0.011
295.2541783	0.076
298.4246851	0.141
322.2378025	0.206
346.6932049	0.272
387.539956	0.338
424.5930571	0.403
488.6261136	0.468
543.3617968	0.534
591.5416081	0.599
662.7939855	0.664
705.8879071	0.730
726.2054064	0.795
779.2813327	0.861
825.2845352	0.926
862.9974701	0.991
850.8254268	1.056
922.3173851	1.122
943.637542	1.187
908.8872424	1.252
964.0092588	1.318
948.9571252	1.383
971.1181303	1.449
941.1816102	1.514
925.6106348	1.579
};  



\end{groupplot}

\end{tikzpicture}

==> Figures/Fig2.tex <==
\begin{tikzpicture}


\node[anchor=north west] at  (-1,0)
{\includegraphics[width=0.7\textwidth]{Fig2.pdf} };


\node (A) at (-0.95, -3.){};
\node (B) at (10.75, -3.){};

\draw[dashed, line width = 1.5,color=black] (A) edge (B);




\node (A) at (5.46, -0.07){};
\node (B) at (5.46, -3.15){};

\draw[-, line width = 1.5,color=blue] (A) edge (B);

\node (A) at (9.12, -0.07){};
\node (B) at (9.12, -3.15){};

\draw[-, line width = 1.5,color=blue] (A) edge (B);


\node (A) at (1.9, -0.07){};
\node (B) at (1.9, -3.15){};

\draw[-, line width = 1.5,color=blue] (A) edge (B);


\node[align=center,color=black,anchor=north west,fill=white,fill opacity=0.2,text opacity=1] at (-.3cm,-3.1cm) {pseudo-bottom};



\end{tikzpicture}
